Subordination of discrete snakes

Motivated by applications in random geometry, we investigate the notion of subordination of snakes in the discrete setup. More precisely, given a random walk $W$ indexed by a tree $T$ and with steps in $\{...,-1,0,1\}$, we consider its subordinate tree obtained by contracting every edge of $T$ that does not lead to a new record of the walk $W$. When the underlying tree $T$ is a Bienaym\'e-Galton-Watson tree, we characterize the distribution of this subordinate tree. In particular, when $T$ has a critical offspring distribution in an $\alpha$-stable domain of attraction with $\alpha\in(1,2]$, and under a light tails assumption on the steps, we prove that the associated subordinate tree is itself a Bienaym\'e-Galton-Watson tree with an offspring distribution in an $\frac{\alpha+1}{2}$-stable domain of attraction. Along the way, we obtain the asymptotic tail of the maximal displacement of the critical branching random walk $W$ in this stable regime, under minimal assumptions. Finally, we use these results to prove scaling limit statements about the subordinate tree.

==> commandes.tex <==


% \RequirePackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\RequirePackage[english]{babel}

\RequirePackage[top=3cm, bottom=3cm, left=3cm, right=3cm, includehead, includefoot, headsep=1.5\baselineskip]{geometry}
\RequirePackage{xspace}
\RequirePackage{amsmath, amssymb, amstext, amsthm, mathtools, mathrsfs, stmaryrd}		% packages des maths
\RequirePackage{hyperref}
\RequirePackage{makeidx}
\RequirePackage{dsfont}					% pour le 1 gras
%\RequirePackage{enumerate}
\RequirePackage[shortlabels]{enumitem}
\setlist[itemize, 1]{label=\textbullet}
\setlist[itemize, 2]{label=--}
\RequirePackage{indentfirst}
\RequirePackage[varg]{pxfonts}
\RequirePackage{graphicx}
\RequirePackage{tikz}
\RequirePackage{xcolor}
\RequirePackage{bbding}
\RequirePackage{wasysym}
\RequirePackage{utfsym} 
\RequirePackage{fontawesome}
\RequirePackage{halloweenmath}
\RequirePackage{pifont}
\RequirePackage{soul} % pour barrer 
\RequirePackage{scsnowman}
\usepackage{bbold}
\usepackage{subcaption}
\usepackage{todonotes}
\usepackage{tcolorbox}

\usepackage[sortcites=true]{biblatex}
\usepackage{csquotes}
\addbibresource{biblio.bib}

\DeclareFontFamily{U}{dancers}{}
\DeclareFontShape{U}{dancers}{m}{n}{<-> dancers}{}

\newcommand{\task}[1]{\todo[color=green!30,inline]{#1}}
\newcommand{\rep}[1]{\todo[color=orange!30,inline]{#1}}

%%%%% RACCOURCIS STYLES DE LETTRES

%%% MATHBB package -> double barre
\usepackage{calrsfs}

\newcommand{\nota}[1]{{\bf \color{red} [#1]}}		% note
\newcommand{\ie}{\textit{i.e. }}
\newtheorem*{rmk}{Remark}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lem}[theorem]{Lemma}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{expl}[theorem]{Example}

\newtheorem{assum}{Assumption}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\renewcommand{\proofname}{Proof}
\newcommand{\A}{\mathbb{A}}
\newcommand{\B}{\mathbb{B}}		% boule
\newcommand{\C}{\mathbb{C}}		% complexes
\newcommand{\D}{\mathbb{D}}		% disque
\newcommand{\E}{\mathbb{E}}		% espérance
\newcommand{\e}{\mathbf{e}}		% espérance
\newcommand{\F}{\mathbb{F}}		% corps à q éléments
\newcommand{\G}{\mathbb{G}}
\renewcommand{\H}{\mathbb{H}}	% quaternions
\newcommand{\I}{\mathbb{I}}
\newcommand{\J}{\mathbb{J}}
\newcommand{\K}{\mathbb{K}}		% corps quelconque
\renewcommand{\L}{L}	% espaces L^p
\newcommand{\M}{\mathbb{M}}
\newcommand{\N}{\mathbb{N}}	
\newcommand{\n}{\mathbf{n}}	% entiers naturels
\renewcommand{\O}{\mathbb{O}}
\renewcommand{\P}{\mathbb{P}}	% proba
\newcommand{\Q}{\mathbb{Q}}		% rationnels
\newcommand{\q}{\mathbf{q}}	
\newcommand{\R}{\mathbb{R}}		% réels
\renewcommand{\S}{\mathbb{S}}	% sphère
\newcommand{\T}{\mathbb{T}}
%\newcommand{\t}{\mathbf{t}}
\newcommand{\U}{\mathbb{U}}		% racines de l'unité
\newcommand{\V}{\mathbb{V}}
\newcommand{\W}{\mathbb{W}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\Y}{\mathbb{Y}}
\newcommand{\Z}{\mathbb{Z}}		% entiers relatifs

%%% MATHCAL -> lettres calligraphiées

\newcommand{\cA}{\mathcal A}		% tribu
\newcommand{\cB}{\mathcal B}		% tribu
\newcommand{\cC}{\mathcal C}	% tribu
\newcommand{\cD}{\mathcal D}
\newcommand{\cE}{\mathcal E}	
\newcommand{\cF}{\mathcal F}		% ensemble des fonctions
\newcommand{\cG}{\mathcal G}	% graphe
\newcommand{\cH}{\mathcal H}	% quaternions, Hilbert
\newcommand{\cI}{\mathcal I}		% idéal
\newcommand{\cJ}{\mathcal J}		% idéal
\newcommand{\cK}{\mathcal K}		% algèbre
\newcommand{\cL}{\mathcal L}		% applications linéaires
\newcommand{\cM}{\mathcal M}	% matrices
\newcommand{\cN}{\mathcal N}	% loi normale
\newcommand{\cO}{\mathcal O}	% O de LANDAU
\newcommand{\cQ}{\mathcal Q}	% O de LANDAU
\newcommand{\cP}{\mathcal P}		% propriété
\newcommand{\cR}{\mathcal R}	% relation
\newcommand{\cS}{\mathcal S}
\newcommand{\cT}{\mathcal T}		% Tribu
\newcommand{\cU}{\mathcal U}	% loi uniforme
\newcommand{\cV}{\mathcal V}
\newcommand{\cW}{\mathcal W}
\newcommand{\cX}{\mathcal X}	
\newcommand{\cY}{\mathcal Y}
\newcommand{\cZ}{\mathcal Z}

%%% MATHSCR -> lettres attachées
\newcommand{\Cs}{\mathscr{C}}	% Cercle
\newcommand{\Hs}{\mathscr{H}}	% Hilbert
\newcommand{\Ks}{\mathscr{K}}
\newcommand{\Ps}{\mathscr{P}}	% propriété
\newcommand{\Ss}{\mathscr{S}}	% système

\newcommand{\1}{\mathds{1}}			% indicatrice
\newcommand{\law}[1]{\text{Law}\left( #1 \right)}			% loi
\newcommand{\dd}{\mathrm{d}}

